Revisiting Actor Programming in C++

The actor model of computation has gained significant popularity over the last decade. Its high level of abstraction makes it appealing for concurrent applications in parallel and distributed systems. However, designing a real-world actor framework that subsumes full scalability, strong reliability, and high resource efficiency requires many conceptual and algorithmic additives to the original model. In this paper, we report on designing and building CAF, the "C++ Actor Framework". CAF targets at providing a concurrent and distributed native environment for scaling up to very large, high-performance applications, and equally well down to small constrained systems. We present the key specifications and design concepts---in particular a message-transparent architecture, type-safe message interfaces, and pattern matching facilities---that make native actors a viable approach for many robust, elastic, and highly distributed developments. We demonstrate the feasibility of CAF in three scenarios: first for elastic, upscaling environments, second for including heterogeneous hardware like GPGPUs, and third for distributed runtime systems. Extensive performance evaluations indicate ideal runtime behaviour for up to 64 cores at very low memory footprint, or in the presence of GPUs. In these tests, CAF continuously outperforms the competing actor environments Erlang, Charm++, SalsaLite, Scala, ActorFoundry, and even the OpenMPI.

==> network-io.tex <==
\section{Message-based Network IO}

When communicating to other services in the network, handling data packets or
byte streams manually is often inevitable.
For this reason, CAF provides \emph{brokers}.
A broker is an event-based actor running in the so-called middleman that
multiplexes asynchronous (socket) IO.
It can maintain any number of acceptors and connections as well as
datagram-oriented wrappers for connectionless protocols.
Since the broker runs in the middleman, implementations should be careful to
consume as little time as possible in message handlers.
Any considerable amount work should outsourced by spawning new actors (or
maintaining worker actors).

The middleman (MM) is a software entity that enables late binding of low-level,
platform-specific communication primitives to platform-independent actors.
It translates network-layer events and byte streams to special-purpose messages
as shown in Listing \ref{lst:brokermsgs}.
Brokers operate on opaque \emph{connection} and \emph{acceptor} handles.
The former are used to identify end-to-end connections while the latter
identifies end endpoint \todo{Frage an die Network Gurus: Guter/richtiger Term?
IdR steckt hinter einem ``endpoint'' ein TCP acceptor socket''} that others can
connect to.

\begin{lstlisting}[caption={Special-purpose messages for
brokers.},label=lst:brokermsgs]
struct new_connection_msg {
  accept_handle source;
  connection_handle handle;
};
struct new_data_msg {
  connection_handle handle;
  std::vector<char> buf;
};
struct connection_closed_msg {
  connection_handle handle;
};
struct acceptor_closed_msg {
  accept_handle handle;
};
\end{lstlisting}

Brokers are spawned using the function \lstinline^spawn_io^ and always use
functor-based implementations capturing the self pointer of type
\lstinline^broker*^.
Since brokers are technology-agnostic, the runtime system of CAF can select the
appropriate communication protocol at runtime.

It is worth mentioning that the runtime implicitly salvages and re-uses
existing buffers.
Brokers run in the context of the MM.
This means that the MM directly calls the message handler of its brokers with a
message containing a \lstinline^new_data_msg^.
The MM uses always the same message, re-writing the contained buffer over and
over again.
As long as the broker does not add a new reference count to this message, no
copy of this buffer will ever be produced due to the copy-on-write
optimization.

\todo{Explain write buffer and configure-read, plus add short example.}

\todo{Add overhead discussion + short evaluation (iperf).}

%For convenience, \lstinline^spawn_io_server^ can be used to spawn a new broker
listening to a local TCP port and \lstinline^spawn_io_client^ can be used to
spawn a new broker that connects to given host and port.
%Brokers receive system messages directly from the middleman whenever an event
on one of it IO handles occurs.
%Those handles are opaque types and do not expose any underlying communication
primitive such as sockets for instance.
%
%Whenever a new incoming connection (identified by the \lstinline^handle^
field) has been accepted for one of the broker's accept handles, it will
receive a \lstinline^new_connection_msg^.
%
%New incoming data is transmitted to the broker using messages of type
\lstinline^new_data_msg^.
%The raw bytes can be accessed as buffer object of type
\lstinline^std::vector<char>^.
%The amount of data, i.e., how often this message is received, can be
controlled using \lstinline^configure_read^.
%It is worth mentioning that the buffer is re-used whenever possible.
%This means, as long as the broker does not create any new references to the
message by copying it, the middleman will always use only a single buffer per
connection.
%
%A \lstinline^connection_closed_msg^ or \lstinline^ acceptor_closed_msg^
informs the broker that one of it handles is no longer valid.

